An Improved Encoder-Decoder Framework for Food Energy Estimation

Dietary assessment is essential to maintaining a healthy lifestyle. Automatic image-based dietary assessment is a growing field of research due to the increasing prevalence of image capturing devices (e.g. mobile phones). In this work, we estimate food energy from a single monocular image, a difficult task due to the limited hard-to-extract amount of energy information present in an image. To do so, we employ an improved encoder-decoder framework for energy estimation; the encoder transforms the image into a representation embedded with food energy information in an easier-to-extract format, which the decoder then extracts the energy information from. To implement our method, we compile a high-quality food image dataset verified by registered dietitians containing eating scene images, food-item segmentation masks, and ground truth calorie values. Our method improves upon previous caloric estimation methods by over 10\% and 30 kCal in terms of MAPE and MAE respectively.

==> review.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 8674
TITLE: An Improved Encoder-Decoder Framework for Food Energy Estimation
AUTHORS: Jack Ma, Jiangpeng He and Fengqing Zhu

----------- Presentation -----------
SCORE: 4 (good)
----------- Innovation -----------
SCORE: 4 (good)
----------- Overall evaluation -----------
SCORE: 3 (borderline paper)
----- TEXT:
In this paper an encoder-decoder framework for food energy estimation is presented. The proposed method outperforms the considered baselines and the dataset used in the experiments will be released to the community. The paper is well-written, the related works section is comprehensive and the purpose of the work is clearly pinned.

- I believe that the reasoning presented in the introduction about the "bottleneck" of image representations is somehow misleading. Although it is true that a food dish may have infinite values of calories, in practice we are hardly interested in a sub-decimal precision of calories estimation and the range of calories for each meal is in the order of thousands. Also, the proposed representation can assume finite values , therefore the recognizable calories values are "bottlenecked" as well.

clarify motivation (emphasize truncation/rounding leads to lost information)

- More information on the number of registered dietitians and on the data collection process should be provided.

clarify what I did commpared to others, provide more specifics, find info on foodinfocus, combine these datasets together
how images captured, how 

- The reference to cGAN in paragraph 4.1.2 is broken.

- Why is section 5.2 named "Main results"? I could not find any other results in sudden sections.

- The number of baselines used for comparison is very small and most methods belong to a single paper ([16]) which dates back to 2 years ago.

in exp section, mention why picked [16] for results in experiemnts (most methods use other types, no monocular, monocular is very limited since it is challenging task, these papers use monocular)

- The ablation study is limited as the only experiment is done by replacing the decoder network. Also, results in Table 2 shows that a ResNet50 backbone network obtains a slightly higher MAE but a consistently lower MAPE. This should be discussed properly and the choice of using the proposed summation decoder in respect to these alternatives must be justified.
two choices
1: validate on encoder greyscale vs tensor
2: further clarify/emphasize why only do abalation study on decoder

summarze observaitons like pretrianed/nonpretrianed, and compare summation with other regresssion decoders. marignal improvement but reqires trainig and stuff, but our decoder is simpler, don't require anything

maybe also clarify mae vs mape and role of these two metrics, which one is better for what

why are performances different for vgg, resanet18, resnet50? resent50 comtians more parameters than resnet18, but achieve siilar results, what does this indicate? incrase model compelxity may not always increase accuracy, this aligns iwth my conclusion

The purpose is sound and the fact the dataset will be made publicly available is a plus, but I find the experimental evaluation of the method and the comparison to existing techniques somehow limited, same for the ablation study. I lean for a borderline rejection of the paper.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 8674
TITLE: An Improved Encoder-Decoder Framework for Food Energy Estimation
AUTHORS: Jack Ma, Jiangpeng He and Fengqing Zhu

----------- Presentation -----------
SCORE: 4 (good)
----------- Innovation -----------
SCORE: 3 (fair)
----------- Overall evaluation -----------
SCORE: 4 (weak accept)
----- TEXT:
In this paper, the authors present an encoder-decoder model designed to predict the energy content (in kcal) of a meal using a single image and its corresponding segmentation mask as inputs. The proposed method, using a single summation as a decoder, outperforms more complex methods that require the training of the decoder.

Although the paper is generally well-structured and concise, there exist a few notable limitations::

-The authors mention that they enhance a previously published dataset. However, key information is missing: how many images did they add, how many dieticians were involved, why did they have to discard data if the dietitian offered the pre-weighed foods to the participants etc.

same thing as reviewer 1

-The authors do not mention the problem of occlusion, i.e., if in a meal image a food component is in front of another food component.


-Figure 4 is not clear. Why are there decimals in the y axis? A barplot could potentially offer clearer representation, where the x-axis corresponds to each meal and the y-axis conveys the error or absolute error of the two approaches.

try to do bar plot, if it look beter then can replace, but make y axis integer

-In table 2 while the results of the authors' methods are in bold, even if they are not the best among the different approaches? 

Also, some discussion should be added about the results (e.g., why pre-trained networks have worse results)

-A reference is missing at paragraph 4.1.2.

In conclusion, I would recommend considering the paper for weak acceptance, as it offers the potential to provide valuable insights to the audience.





notes to self:

double check references, make sure they are accurate
